Collaborative Design for Job-Seekers with Autism: A Conceptual Framework for Future Research

The success of employment is highly related to a job seeker's capability of communicating and collaborating with others. While leveraging one's network during the job-seeking process is intuitive to the neurotypical, this can be challenging for people with autism. Recent empirical findings have started to show how facilitating collaboration between people with autism and their social surroundings through new design can improve their chances of employment. This work aims to provide actionable guidelines and conceptual frameworks that future researchers and practitioners can apply to improve collaborative design for job-seekers with autism. Built upon the literature on past technological interventions built for supporting job-seekers with autism, we define three major research challenges of (1) communication support, (2) employment stage-wise support, and (3) group work support. For each challenge, we review the current state-of-the-art practices and possible future solutions. We then suggest future designs that can provide breakthroughs from the interdisciplinary lens of human-AI collaboration, health services, group work, accessibility computing, and natural language processing.

==> sections/03_problemspace_old.tex <==
\section{Research in Collaborative Job-seeking for People with Autism}

In laying out the main directions in our framework, we collected noteworthy findings from the three types of literature: the survey papers related to intervention for job-seekers with autism (e.g., ~\cite{ezerins2023autism, khalifa2020workplace, Kim_Crowley_Lee_2022, nicholas2015vocational}), (2) empirical papers that provide insights into how people with autism leverage technology to collaborate in seeking jobs (e.g., ~\cite{dillahunt2021implications, dillahunt2016designing, ara2024collaborative}), technical papers that propose intervention for improving job-seeking experience for people with autism, but not necessarily use social approach (e.g.,~\cite{adiani2022career, pouliot2017tool} ).
In analyzing the papers, the first authors coded the scoped paper regarding any noteworthy empirical insights and opinions. 
Using these codes as an initial resource, every author participated in affinity diagramming and theme-generation process following qualitative research~\cite{saldana2015coding, layder1998sociological}. 
In shaping our final themes, each of the authors built their structure based on their expertise and compared the structures to identify commonalities and discrepancies
The discussion continued multiple rounds until every author reached a consensus. 
Consequently, we identified the three directions---Communication Support, Employment Stage-wise Support, and Group work support---as imminent and important problems that can yield practical impact on the collaborative design for job-seekers with autism. 

\subsection{Communication Support} 

\paragraph{Background and State-of-the-Art}

One of the most common challenges discussed in the past literature is the different styles of using languages between people with autism and neurotypicals. In particular, people with autism tend to be literal thinkers whereas neurotypical languages use various implicit language devices, such as abstraction, metaphor, mapping, sarcasm, or euphemisms.
Past research has identified such communication breakdown as a core reason for people with autism to be not successful in the employment market~\cite{lorenz2016autism, ara2024collaborative}
Some communication challenge examples featured in the previous literature include: interpreting implicit languages such as metaphors, analogies, and idioms in the intended way; and handling casual topics (i.e. small talks unrelated to the search); adjusting to blunt language and level of formality depending on the conversational context; and taking turns (i.e., controlling conversational flow without hyper-focusing on a topic of interest or balancing the volume of conversation between two people).
A recent study has found how such different styles of using language can cause unsuccessful outcomes in every stage of job-seeking; when reading job calls, asking for details about jobs to hiring managers, conducting interviews, and negotiating the offer~\cite{ara2024collaborative}.

Mitigating the communication gap is the core to building up social skills related to their career~\cite{ezerins2023autism}.
Therefore, it is imperative to devise technological intervention to mitigate the gap between literal language and contextual language ~\cite{nicholas2015vocationa}. 
Such language translation is relatively scarce in literature but started to appear.
For instance, Pouliot et al. devised a communication supporting method using ``communication story''~\cite{pouliot2017tool}. 

\paragraph{Research Directions}

In developing the new intervention for conversational support, the requirements will be different between the following two cases of \textit{conversational decoding}---people with autism understanding neurotypical language---and \textit{encoding}---people with autism adjusting neurotypical language. In decoding, it is crucial to develop a way to detect the implicit use of language and translate it to the explicit one. 
NLP techniques such as XXX - XXX - XXX - XXX can be applied in developing the encoding scenarios. 
In encoding, language style transfer and tone changing can be useful. One aspect that makes people with autism find it difficult to initiate cold communication is closely associated with their anxiety of being perceived as ``rude'' or ``unfeeling''~\cite{ara2024collaborative}. In many cases, people with autism get help from their surroundings to check the ``tone and manner'' of their writing style~\cite{ara2024collaborative}. While social surroundings can proofread writings and guide people with autism to formulate answers to expected interview questions, providing such feedback across the whole period of the job-seeking process from scratch can be physically and mentally exhausting. Therefore, designing intelligent interventions that can reduce the effort of social surroundings will be perceived as useful. 

In developing such intelligent group-AI collaboration interfaces in both directions of conversation, we list a couple of more challenges.
To build AI models that can be specifically accurate for conversational encoding and decoding, characterizing the common cases of misalignment using numerous cases of conversation made in employment contexts is essential. 
Such case collection and classification are under the domain of data annotation. 
There has been extensive research in interactive data annotation~\cite{choi2019aila}. 
However, few approaches have been proposed for making the annotation efficient and effective in job-seeking scenarios for people with autism.
In addition, in developing interactive user interfaces used for conversational encoding and decoding, strictly applying a human-centered and/or participatory methodology by closely communicating with multi-stakeholders involved in the problem (i.e., people with autism and various social surrounding groups) can increase the chance of building the intervention that is perceived as practical, useful, and be adopted in situ to create impact. 

\subsection{Employment Stage-wise Support}

\paragraph{Background and State-of-the-Art}
Employment is a process with multiple stages.
While such a process can be challenging for everyone, numerous articles explain why and how each stage can impose even more severe challenges on people with autism than their neurotypical peers~\cite{ara2024collaborative}.
From the moment of reading a job advertisement to negotiating an offer, each stage in the employment process can be daunting to people with autism.
A few empirical studies identified the importance of step-by-step, end-to-end support such as writing cover letters, resumes, and intelligent tutoring~\cite{dillahunt2021implications}.

In terms of state-of-the-art, \textit{DreamGig} helps underserved job-seekers find job openings that align with their career goal and supports them in identifying skills they need to achieve to reach their dream jobs~\cite{dreamgig}.
there have been another line of interactive systems built for supporting employment stages, such as \textit{Review-Me} that supports resume editing and \textit{Interview4} that elicit feedback for interviews from volunteers~\cite{dillahunt2021implications}.
While there are not many technological interventions specifically focusing on job-seekers with autism as a user group, past studies' results imply how developing a dedicated feature specifically focusing on stage-wise support can improve the performance of job-seekers with autism.

\paragraph{Research Directions}

Literature shows how people with autism can easily be distracted or feel hardship in prioritizing employment-related tasks~\cite{ara2024collaborative}. 
Several challenges occur during the employment process, those are related to the way in which the job is presented, regarding the description of the position and the required qualifications of the candidate. Other issues emerge due to the numerous steps required to prepare the materials, manage the scheduling, and go through a selection process as detailed below.


\textbf{Searching job ads}:
First of all, it is crucial to help people with autism to easily narrow down job calls based on what they are looking for.
There exists a misalignment between what people with autism commonly look for and what current ``go-to'' search tools are providing.
To people with autism, environmental factors, such as noise level, team-related activity factors, such as the frequency and intensity of communication for finishing up their main responsibility, and the organization's culture about Diversity, Equality, and Inclusion (DEI)---either they put the DEI statement in their job ads as ``boilerplate'' or the statement truly represent their culture and a company can work flexibly with their employees to accommodate their needs---become crucial factors~\cite{khalifa2020workplace}. 
Additionally, some positions require drastic life changes, such as re-location. However, a change in routine is particularly challenging for people with autism.
While many search tools---or the majority of job advertisements---don't provide these factors, one aspect that future design can consider is to identify how to efficiently categorize numerous job calls based on such factors.
The factors that job-seekers with autism are looking for can be diverse and change.
Interactive searching environments that flexibly accommodate their criteria can significantly reduce their effort. 

\textbf{Reading job ads}:
Developing a reading environment that minimizes the chance of long reading of text---exhausting the attention span of people with autism or introducing unwanted misinterpretation---can provide aid. 
Job ads often describe roles and responsibilities purposefully vague to invite a large number of candidates.
They also provide a long text to cover every aspect about the new job opportunity.
That, summed with people with autism's characteristics of ``literal thinkers'', many job ads make them hesitate to apply when they feel like not all job requirements are being sufficiently met.
They can also be easily distracted or lose focus due to the long length and implicit language. 
In developing an autism-friendly environment, recent advances in large AI models can provide several solutions that can meaningfully improve job seekers with autism's job search-related productivity. 
For instance, modern summarization and simplification models can convert job ads to less lengthy forms written with autism-friendly language.
Text-based Question Answering techniques can prevent people with autism from retaining information in their brains and allow them to gradually understand step by step using their preferred order of questions.

\textbf{Writing cover letter, resume, and preparing materials:}
Finetuning cover letters and resumes can be also challenging for job-seekers with autism especially because they may likely apply for multiple jobs simultaneously. 
An interactive co-editing design between people with autism, an AI agent, and their social surroundings that can easily convert their findings from job ads reading into cover letters and resume editing can become useful in such a scenario.
In addition, the preparation of the job materials can be overwhelming for job seekers with autism.
Unfortunately, in many cases, the required materials for application are not presented in a structured way with templates.
Additionally, not describing the expected contents and specific steps entailed in the hiring process incurs anxiety during the application process.
Not only do they face challenges preparing and submitting the documents required, but also contact the HR personnel to seek help and interview through calls or in-person.
Designing, developing, and evaluating intelligent agents who can support people with autism and their social surroundings to handle these difficulties can help job seekers with autism to be better prepared.

\textbf{Conducting interviews:}
For job seekers with autism, participating in the interview is one of the most challenging steps in the hiring process.
Some candidates may also face challenges due to required improvisation when the interview questions are not known upfront.
For them, it is hard to project themselves into situations that are not yet experienced (imagined scenarios).
On top of the unanticipated questions, the fact of making conversation with an unknown group of people adds to the challenge.
In the case where a script with interview questions is not available, developing the mock interview or shadow interview environment that enables (1) people with autism to be exposed to a variety of questions related to the job while (2) social surroundings can easily review and provide their comments can help them.
Also, it is important to help people with autism understand when to take turns, estimating what can be the right volume of answers to fit within the interview timeframe can be important to facilitate their communication flow. 
Moreover, for the candidate to feel comfortable, it is recommended to help them understand when to take breaks.
In helping them learn the aspects mentioned above, current research in using wearable devices that can measure their anxiety level in real time or applying devices that provide immersive environments can provide practical future interventions. Gamification design blended with multimodal guidance of providing unique visual and audio feedback depending on how people with autism answer the question or providing cues for time-related information can make a difference.

\textbf{Networking and communication with employers}
Finally, devising a future networking design that people with autism can leverage in reaching out to volunteers can be helpful. 
However, volunteering in a job-seeking situation expects longitudinal and heavy commitment.
The networking feature should carefully consider why both parties can readily agree to work together. 
In doing so, recent research shows that people with autism have a strong preference for seeking people who have commonalities in the neurodiverse spectrum and cultural fit.

%Say something 

\subsection{Groupwork Support}

\paragraph{Background and State-of-the-Art}

Groupwork is the subdomain of CSCW where the aim is to understand how a group of people work together on a certain task using technology in different modes of situations; working synchronously or asynchronously, and at the same space or in a distributed manner~\cite{cook2005illuminating}. 
As one of the most social beings on Earth~\cite{kraut2002aristotle}, humans can collaborate on almost any task under the shared vision. 
While one could imagine that groupware can aid groups easily, Grudin's early work in CSCW has identified that boosting a group's productivity using socialware is extremely challenging~\cite{grudin1988cscw, grudin1994groupware}.
Despite the challenges entailed in designing successful groupware, decades of research have found how groupwork support can create a tremendous impact on several domains that would have been not possible otherwise~\cite{rama2006survey}, enabled advancing democracy, motivating DEI, regulating disinformation, realizing international scientific collaboration, and more~\cite{thaw2008cope, hong2018collaborative}.

As we briefly mentioned in Section 2, we found few studies that systemically leverage groupwork as an intervention to facilitate the job-seeking process for people with autism. 
However, recent studies started to show evidences that how groupwork can be a promising direction as a new intervention. 
For instance, using better technology, one study found how underresourced job-seekers can make a difference on their outcomes with career advisors~\cite{dillahunt2021implications}.
With a more productivity-centered groupware design, career specialists can support more people who are in need of help~\cite{lorenz2016autism}. 
This may contribute to making professionals more available to a broader population of autism who could receive benefits~\cite{dillahunt2021implications}.
Another study found varying contexts that tell us how people with autism collaborate with their social surroundings, describing various technological barriers that blcok them from collaboration~\cite{ara2024collaborative}.

\paragraph{Research Directions}

Supporting group collaboration using technology is challenging because any matters that happen between humans are context-dependent and change every moment.
Since technology is especially effective for handling similar and repetitive activities, Ackerman coined his notion of ``social-technical gap'' which explains why we may never be able to resolve problems that require social collaboration using technology~\cite{ackerman2000intellectual}.
In recent years, advances in large language models and intelligent agents started to demonstrate meaningful breakthroughs.
Therefore, this section will explain the directions of AI-driven collaboration support that could lead to a successful collaborative design for job seekers with autism.

\textbf{AI agents that help executive planning and multi-tasking}:
One of the most challenging aspects of job-seeking for people with autism is to cope with handling multiple job opportunities that have strict deadlines. 
Once they focus on one task, they may easily fall into time-blindness and be late on the interview or miss deadlines~\cite{ara2024collaborative}.
Handling the deadlines, and helping the group to understand what will come and what needs to be done is a complex task that intelligent agents can support human groups. 

\textbf{AI agents that can soften between-member dynamics and relationships}:
Conflict resolve is one of the most challenging aspects in groupwork~\cite{miranda1993impact}.
A variety of  conflict can arise while working on a high stake task with impact, such as job-seeking. 
There are several reasons that conflict can arise; caring other members can be seen as meddling, asking of information on each member's activity can be perceived as violating privacy. 
Managing disagreement on the decision can be also important topic~\cite{harris2018small}. 

\textbf{AI that manage volume of communication and coordinate dependencies for reduced work}:
Finally, the core competency of groupware is to enable the group to achieve their goal in a high quality using reduced effort. 
One downside of groupwork is the necessity of communicating with others to synchronize their situational and group awareness~\cite{hong2018collaborative}. 
In many cases, they must coordinate their group work to manage dependencies between activities~\cite{malone1994interdisciplinary}.
Understanding how to effectively resolve such activities using the AI-empowered agent can create useful solutions.
One of the most challenging aspects of job-seeking for people with autism is to cope with handling multiple job opportunities that have strict deadlines. 
Once they focus on one task, they may easily fall into time-blindness and be late on the interview or miss deadlines~\cite{ara2024collaborative}.
Handling the deadlines, and helping the group to understand what will come and what needs to be done is a complex task that intelligent agents can support human groups. 

==> sections/999_raythoughts.tex <==
how job interview a process can impose more challenges on people with autism~\cite{flower2021barriers}

>> designing/adopting the new socialware entails understanding the context of use thus empirical study required~\cite{ehrlich1987strategies}

>> challenges in designing socialware~\cite{grudin1988cscw}
>> challenges in designing socialware~\cite{grudin1994groupware}

>> groupware conflict resolve~\cite{miranda1993impact}

>> small group decision making~\cite{harris2018small}

>> coordination - managing dependencies between activities -impoact of it~\cite{malone1994interdisciplinary}

>> social-technical gap~\cite{ackerman2000intellectual} 
>> mitigating social-techical gap is the fundamental challenge in cscw...
>> flexible, nuanced, and contextual awareness, division of labor, persistence are important. searchtogether~\cite{morris2007searchtogether}

https://pressbooks.pub/smallgroup/chapter/decision-making-in-groups/
``advantage of drawing from the experiences and perspectives of a larger number of individuals. Hence, the ideas have the potential to be more creative and lead to a more effective decision.''

>> group decision-making~\cite{hong2018collaborative, }
>> collaborative informaton-seeking~\cite{hong2019design}
>> structures that enable and constrain the future action based on social collaboration~\cite{scott1992microlevel}
>> collaborative sequencing~\cite{kim2021supporting}
>> infovis collaborative visual analytics~\cite{heer2007design}



>> barriers in seeking jobs ~\cite{lorenz2016autism}
>> external help can be useful in seeking jobs~\cite{lorenz2016autism}
>> Communication and human interaction is a problem~\cite{lorenz2016autism}
>> "formality problem": organizational culture is a challenge - not enough accomodation~\cite{lorenz2016autism}
>> external help can be - external institutions / private~\cite{lorenz2016autism}
>> external help is useful, but hard to practice (less than <15\%)~\cite{lorenz2016autism}

>> pre-employment: transition from education job search - a known impediment on barrier to employment = navigating~\cite{ezerins2023autism}
>> Individuals often experience a dramatic reduction in formal support upon exiting secondary school, transitions to employment are likely to be especially difficult and precarious~\cite{ezerins2023autism}


>> social skill helps~\cite{ezerins2023autism}


>> job interview very difficult for people with autism~\cite{ezerins2023autism}

>> Annabi and Locke reviewed the literature on autism employment and synthesized it into a theoretical framework to study IT workplace readiness, and also revealed that barriers and opportunities in the IT workplace are influenced by individual differences, individual coping methods, autism employment programs, and neurotypical attitudes towards people with autism and knowledge about autism~\cite{annabi_locke_2019}.
>> Technological intervention can make differences in autism task performance~\cite{khalifa2020workplace}

>> working with career advisors can boost the odds for being employed especially for marginalized population~\cite{dillahunt2021implications}

>> but career advisors are relatively inaccessible resource for many people with autism~\cite{dillahunt2021implications}

>> Social support is a significant boost for those marginalized/has economic constraints.  ~\cite{dillahunt2021implications}

>> help underserved population to recognize the skills they need to learn recognize their skill sets and find job openings that match with their skills~\cite{dreamgig}.



>> intervention: design for disadvantaged job seekers: resume feedback from volunteers~\cite{dillahunt2016designing}

>> Review-Me resume feedback tool and Interview4 interview feedback tool~\cite{dillahunt2020positive}

>> step-by-step support ii.e., writing cover letters, resume, intelligent tutoring will be useful~\cite{dillahunt2021implications}

>> autism - VR device to prepare interviews, helping them to reduce anxiety~\cite{adiani2022career}

>> survey: Technology intervention: watching instructional video, simulated mock interview, feedback~\cite{Kim_Crowley_Lee_2022}


>>  survey: (1) community placement and job coaching and media and technology–based augmentative tools~\cite{nicholas2015vocational}


>> The literature is limited in volume and quality of methodology, yet emerging constructs are promising in introducing the utility of vocational resources~\cite{nicholas2015vocational}

>> Future studies are needed that assess the role of peer relationships in fostering vocational success~\cite{nicholas2015vocational}



>> among 22,878 papers examined - scarce of research for adults with autism 3974 articles identifying an ASD intervention, 501 studies (12.6\%) targeted participants 18 years of age or older. only 10 papers focused on supporting jobs. \cite{nicholas2015vocational}

>> a tool for supporting communication - during work (after employment" using "communication story"~\cite{pouliot2017tool}
